Reward Signal Design for Autonomous Racing

Reinforcement learning (RL) has shown to be a valuable tool in training neural networks for autonomous motion planning. The application of RL to a specific problem is dependent on a reward signal to quantify how good or bad a certain action is. This paper addresses the problem of reward signal design for robotic control in the context of local planning for autonomous racing. We aim to design reward signals that are able to perform well in multiple, competing, continuous metrics. Three different methodologies of position-based, velocity-based, and action-based rewards are considered and evaluated in the context of F1/10th racing. A novel method of rewarding the agent on its state relative to an optimal trajectory is presented. Agents are trained and tested in simulation and the behaviors generated by the reward signals are compared to each other on the basis of average lap time and completion rate. The results indicate that a reward based on the distance and velocity relative to a minimum curvature trajectory produces the fastest lap times.

==> BlockDiagrams/nav_arch.tex <==

\usetikzlibrary{shapes.geometric, arrows}

\usetikzlibrary{shapes, shadows, arrows, arrows.meta}

\tikzstyle{empty} = [rectangle, rounded corners, draw=white, minimum height = 0.2cm, minimum width=0.2cm]
\tikzstyle{block} = [rectangle, rounded corners, draw=black, minimum height = 1cm, minimum width=2cm]
\tikzstyle{mysum} = [circle, draw=black]


\tikzstyle{arrow} = [thick, ->, >=stealth]

% \begin{document}


\begin{tikzpicture}[node distance=2cm]

    \node (base) [empty] {};
    \node (b2) [empty, below of=base, yshift=0.5cm] {};
    \node (pf) [block, right of=base, xshift=0.4cm] {Path Follower};
    \node (t_base) [empty, above of=pf, yshift=-0.5cm] {};
    \node (nn) [block, right of=pf, xshift=1cm] {Neural Network};
    % \node (sum) [mysum, right of=pf, xshift=3cm] {};
    \node (b3) [empty, right of=nn, xshift=1cm] {};
    
    
    \draw[arrow] (t_base) -- (pf);
    \draw [arrow] (pf) -- (nn);
    \draw [arrow] (base) -- (pf);
    \draw [arrow] (nn) -- (b3);
    
    \node[align=left] at (1.8, 1) {Global \\ Plan};
    \node[align=left] at (0.5, -0) {Vehicle \\ state};

    \node[align=left] at (7.8, -0.6) {Modified \\ references};

\end{tikzpicture}

==> BlockDiagrams/planningHeirarchy.tex <==
% \documentclass{article}
% \documentclass[12pt, float=false, crop=true]{standalone}

\tikzstyle{empty} = [rectangle, rounded corners, draw=white, minimum height = 1cm, minimum width=2cm]
\tikzstyle{block} = [rectangle, rounded corners, draw=black, minimum height = 1cm, minimum width=2cm]
\tikzstyle{dash_block} = [rectangle, square corners, draw=black, ]

\tikzstyle{arrow} = [thick, ->, >=stealth]

% \begin{document}

% \footnotesize

% Define distances
% \def\blockheight{2.5em}
% \def\blockwidth{2.5em}
% \def\nodesep{4*\blockwidth}

\resizebox{0.46\textwidth}{!}{
    \begin{tikzpicture}[node distance=2cm]
    
        \node (Gplan) [block] {Global Planner};
        \node (map) [empty, left of=Gplan, xshift=-1cm] {Environment Map};
        \node (Lplan) [block, below of=Gplan] {Local Planner};
        \node (c_sys) [block, right of=Lplan, xshift=1.5cm] {Control System};
        \node (sensors) [block, left of=Lplan, xshift=-1cm] {Perception};
        \node (vehicle) [block, below of=Lplan] {Vehicle};
        
        \draw [arrow] (Gplan) -- (Lplan);
        \draw [arrow] (map) -- (Gplan);
        \draw [arrow] (sensors) -- (Lplan);
        \draw [arrow] (Lplan) -- (c_sys);
        \draw [arrow] (c_sys) |- (vehicle);
        \draw [arrow] (vehicle) -| (sensors);
    
    % \draw[dashed] (1,1) -- (1, 5);
    % \draw[dashed] (1,1) -- (4,1);
    % \draw[dashed] (4,1) -- (4,5);
    % \draw[dashed] (1,5) -- (4,5);
    
    
    \end{tikzpicture}
}

% \end{document}

==> BlockDiagrams/semi_gen.tex <==

\usetikzlibrary{shapes.geometric, arrows}

\usetikzlibrary{shapes, shadows, arrows, arrows.meta}

\tikzstyle{empty} = [rectangle, rounded corners, draw=white, minimum height = 0.2cm, minimum width=0.2cm]
\tikzstyle{block} = [rectangle, rounded corners, draw=black, minimum height = 1cm, minimum width=2cm]
\tikzstyle{mysum} = [circle, draw=black]


\tikzstyle{arrow} = [thick, ->, >=stealth]

% \begin{document}


\begin{tikzpicture}[node distance=2cm]


    
    \node (base) [empty] {};
    \node (b2) [empty, below of=base, yshift=0.5cm] {};
    \node (pf) [block, right of=base, xshift=0.4cm] {Path Follower};
    \node (t_base) [empty, above of=pf, yshift=-0.5cm] {};
    \node (nn) [block, right of=pf, xshift=1cm] {Neural Network};
    \node (sum) [mysum, right of=pf, xshift=3cm] {};
    \node (b3) [empty, right of=nn, xshift=1cm] {};
    
    \node (sc) [block, below of=nn] {Speed Calculator};
    
    \draw[arrow] (t_base) -- (pf);
    \draw [arrow] (pf) -- (nn);
    \draw [arrow] (base) -- (pf);
    \draw [arrow] (nn) -- (b3);
    \draw [arrow] (pf) -- (nn);
    \draw [arrow] (nn) -- (sum);
    \draw [arrow] (pf) |- (sc);
    \draw [arrow] (sc) -| (sum);
    \draw [arrow] (nn) -- (sc);
    
    \node[align=left] at (1.8, 1) {Global \\ Plan};
    \node[align=left] at (0.5, -0) {Vehicle \\ state};

    \node[align=left] at (7.8, 0.6) {References};

    \node at (6.9, 0.2) {$+$};
    \node at (7.2, -0.5) {$+$};

\end{tikzpicture}

==> Graphs/dis_sweep.tex <==

% \documentclass[12pt, float=false, crop=true]{standalone}
% \usepackage{import}
% \usepackage{tikz}
% \usepackage{pgfplots}
% \pgfplotsset{compat = newest}

% \begin{document}

\begin{tikzpicture}
	\begin{axis}
		[name=plot,width=.48\textwidth, height=4cm,
		xmin=0, xmax=2.8,
		ymin=50, ymax=120,
		grid=major,
		grid style=dashed,
		xlabel={Time Punishment Per Step ($m_\text{t}$)},
		ylabel={Lap Time},
		legend ]
		
		\pgfplotstableread[col sep=comma,]{Graphs/test_time_sweep.csv}{\table}
		
		\addplot[color=blue, ultra thick] table[x={x}, y={y1}]{\table};
		\addlegendentry{Time Taken}
		\addplot[color=red, ultra thick] table[x={x}, y={y2}]{\table};
		\addlegendentry{Completion \%}
		
		
		% plot lines
% 		\addplot[color=blue, ultra thick] table[col sep=comma]{Graphs/test_time_sweep.csv};
% 		\addplot[color=red, thick] table[col sep=comma]{Graphs/test_time_sweep.csv};
% 		\addplot[color=blue, ultra thick] table[col sep=comma]{Data/TrainingData.csv};
		\label{time_sweep_plot}
	
	\end{axis}
\end{tikzpicture}

% \end{document}

==> Imgs/MinCurve.tex <==
%% Creator: Inkscape inkscape 0.92.3, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'MinCurve.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{508.87194189bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.80289352)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{MinCurve1.pdf}}%
  \end{picture}%
\endgroup%


==> Imgs/NavToRace.tex <==
%% Creator: Inkscape inkscape 0.92.3, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'NavToRace.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{329.7516542bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.66749256)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{NavToRace1.pdf}}%
  \end{picture}%
\endgroup%


==> Imgs/ObsAvoid.tex <==
%% Creator: Inkscape inkscape 0.92.3, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'ObsAvoid.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{218.19293165bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,1.00424392)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{ObsAvoid1.pdf}}%
  \end{picture}%
\endgroup%

